The Bolocam Galactic Plane Survey. VII. Characterizing the Properties of Massive Star-Forming Regions

We present the results of a GBT survey of NH3(1,1), (2,2), (3,3) lines towards 631 Bolocam Galactic Plane Survey (BGPS) sources at a range of Galactic longitudes in the inner Galaxy. We have detected the NH3(1,1) line towards 72% of our targets (456), demonstrating that the high column density features identified in the BGPS and other continuum surveys accurately predict the presence of dense gas. We have determined kinematic distances and resolved the distance ambiguity for all BGPS sources detected in NH3. The BGPS sources trace the locations of the Scutum and Sagittarius spiral arms, with the number of sources peaking between Galactocentric radii of 4-5 kpc. We measure the physical properties of each source and find that depending on the distance, BGPS sources are primarily clumps, with some cores and clouds. We have examined the physical properties as a function of Galactocentric distance, and find a mean gas kinetic temperature of 15.6 K, and that the NH3 column density and abundance decrease by nearly an order of magnitude between Galactocentric radii of 3 - 11 kpc. Comparing sources at similar distances demonstrates that the physical properties are indistinguishable, which suggests a similarity in clump structure across the Galactic disk. We have also compared the BGPS sources to criteria for efficient star formation presented independently by Heiderman et al. and Lada et al., and massive star formation presented by Kauffmann et al. 48% of our sample should be forming stars (including massive stars) with high efficiency, and 87% contain subregions that should be efficiently forming stars. Indeed, we find that 67% of the sample exhibit signs of star formation activity based on an association with a mid-IR source.

==> tab4.tex <==

\begin{deluxetable*}{rcccccccccccc}
\tabletypesize{\scriptsize}
\tablewidth{0pt}
\tablecaption{\label{nh3_props}Observed NH$_{3}$ Properties}
\tablehead{
\colhead{ID} & \colhead{RA} & \colhead{Dec} & \colhead{$V_{LSR}$} & \colhead{$\sigma_{Vlsr}$} & \colhead{\tmb(1,1)} & \colhead{$W$(1,1)} & \colhead{\tmb(2,2)\tablenotemark{b}} & \colhead{$W$(2,2)\tablenotemark{b,c}} & \colhead{\tmb(3,3)\tablenotemark{b,c}} & \colhead{$W$(3,3)\tablenotemark{b,c}} & \colhead{\tmb(4,4)\tablenotemark{b,c}} & \colhead{$W$(4,4)\tablenotemark{b,c}} \\                    
\colhead{Number\tablenotemark{a}} & \colhead{(J2000)} & \colhead{(J2000)} & \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)} & \colhead{(K)} & \colhead{(K km s$^{-1}$)} & \colhead{(K)} & \colhead{(K km s$^{-1}$)} & \colhead{(K)} & \colhead{(K km s$^{-1}$)} & \colhead{(K)} & \colhead{(K km s$^{-1}$)} 
}
\startdata
1307 & 18 02 30.0 & -22 28 06.9 &  32.63 (0.03) & 0.94 (0.03) & 0.85 (0.10) &  6.08 (0.20) & $<$ 0.35 & $<$ 0.97 & $<$  0.39 & $<$ 0.95 & \nodata & \nodata \\ 
1309 & 18 01 00.5 & -22 15 48.5 &   8.16 (0.06) & 0.94 (0.06) & 0.39 (0.09) &  3.21 (0.18) & $<$ 0.35 & $<$ 0.97 & $<$  0.39 & $<$ 0.98 & \nodata & \nodata \\ 
1310 & 18 02 47.8 & -22 26 03.3 & 122.87 (0.03) & 0.60 (0.02) & 0.75 (0.09) &  4.08 (0.18) & $<$ 0.35 & $<$ 0.86 & $<$  0.38 & $<$ 0.83 & \nodata & \nodata \\ 
1311 & 18 03 15.0 & -22 27 09.7 & 153.30 (0.01) & 0.80 (0.01) & 2.54 (0.10) & 19.31 (0.21) & 1.38 (0.09) &  5.88 (0.19) & 1.02 (0.10) &  7.09 (0.19) & \nodata & \nodata \\
1313 & 18 02 45.3 & -22 21 46.8 &  -0.71 (0.04) & 0.77 (0.04) & 0.63 (0.09) &  3.94 (0.19) & $<$ 0.35 & $<$ 0.92 & $<$  0.37 & $<$ 0.88 & \nodata & \nodata \\ 
1314 & 18 03 11.9 & -22 24 32.5 & 154.02 (0.01) & 0.97 (0.01) & 3.38 (0.11) & 28.53 (0.23) & 2.07 (0.09) & 10.59 (0.20) & 1.60 (0.10) & 12.32 (0.20) & \nodata & \nodata \\
1316 & 18 03 31.5 & -22 26 48.4 & 152.52 (0.00) & 0.63 (0.00) & 3.93 (0.10) & 24.58 (0.20) & 2.09 (0.09) &  7.47 (0.18) & 1.19 (0.09) &  6.53 (0.17) & \nodata & \nodata \\
1317 & 18 03 26.8 & -22 25 16.1 & 154.55 (0.02) & 1.01 (0.02) & 1.26 (0.10) & 10.45 (0.21) & 0.48 (0.09) &  2.49 (0.20) & $<$ 0.38 & $<$ 0.96& \nodata & \nodata \\
1320 & 18 02 46.6 & -22 12 17.7 &  18.11 (0.03) & 0.76 (0.03) & 0.75 (0.09) &  4.24 (0.18) & $<$ 0.34 & $<$ 0.90 & $<$  0.38 & $<$ 0.89 & \nodata & \nodata \\ 
1322 & 18 03 23.7 & -22 07 45.9 &   0.26 (0.00) & 0.42 (0.00) & 3.00 (0.09) & 15.52 (0.16) & 1.08 (0.09) &  2.12 (0.15) & $<$ 0.38 & $<$ 0.74& \nodata & \nodata
\enddata \\
\tablecomments{Errors are given in parentheses.  The full table is available in the online journal.}
\tablenotetext{a}{B, C, D, and E denote multiple ammonia pointings that fall within a single 1.1 mm source.}
\tablenotetext{b}{Upper-limits are $T_{mb} < 4\sigma$ and $W < 5\sigma \Delta v  \sqrt{N}$, where $\sigma$ is the rms noise, $\Delta v$ is the width of a single channel in velocity, and $N$ is the number of pixels over which the average RMS was calculated.}
\tablenotetext{c}{\nodata denotes sources that were not observed in the given transition.}
\end{deluxetable*}


